Geometry Image Diffusion: Fast and Data-Efficient Text-to-3D with Image-Based Surface Representation

Generating high-quality 3D objects from textual descriptions remains a challenging problem due to computational cost, the scarcity of 3D data, and complex 3D representations. We introduce Geometry Image Diffusion (GIMDiffusion), a novel Text-to-3D model that utilizes geometry images to efficiently represent 3D shapes using 2D images, thereby avoiding the need for complex 3D-aware architectures. By integrating a Collaborative Control mechanism, we exploit the rich 2D priors of existing Text-to-Image models such as Stable Diffusion. This enables strong generalization even with limited 3D training data (allowing us to use only high-quality training data) as well as retaining compatibility with guidance techniques such as IPAdapter. In short, GIMDiffusion enables the generation of 3D assets at speeds comparable to current Text-to-Image models. The generated objects consist of semantically meaningful, separate parts and include internal structures, enhancing both usability and versatility.

==> figures/gim_separable_objects/figure.tex <==
\resizebox{\linewidth}{!}{
\begin{tikzpicture}% First column with two images
\node[inner sep=0pt] (image11) at (0,0) {\includegraphics[width=3cm]{figures/gim_separable_objects/images/gusnlinger_pistol.png}};

% Second column with one image
\node[inner sep=0pt] at (3, 0) (image21) {\includegraphics[width=3cm]{figures/gim_separable_objects/images/gusnlinger_pistol_sep.png}};

\end{tikzpicture}
}


==> figures/triangulation.tex <==
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[
    vertex/.style={circle,fill=AccentBlue,inner sep=1.5pt},
    edge/.style={thick,draw=AccentBlue},
    label/.style={font=\small\sffamily}
]
% Define custom colors based on the previous scheme
\definecolor{PrimaryBlue}{HTML}{B0D4E5}
\definecolor{AccentBlue}{HTML}{8ABCD1}
\definecolor{NeutralBackground}{HTML}{F5F5F5}

% Create a 4x4 grid of points
\foreach \i in {0,...,3} {
    \foreach \j in {0,...,3} {
        \node[vertex] (v\i\j) at (\i,\j) {};
    }
}
\begin{scope}[on background layer]
% Draw and fill triangles with random diagonals
\foreach \i in {0,...,2} {
    \foreach \j in {0,...,2} {
        % Randomly decide the direction of the diagonal
        \pgfmathparse{int(random(0,1))}
        \ifnum\pgfmathresult=0
            % Diagonal from top-left to bottom-right
            \fill[PrimaryBlue] (v\i\j.center) -- (v\the\numexpr\i+1\relax\j.center) -- (v\i\the\numexpr\j+1\relax.center) -- cycle;
            \fill[AccentBlue] (v\the\numexpr\i+1\relax\the\numexpr\j+1\relax.center) -- (v\the\numexpr\i+1\relax\j.center) -- (v\i\the\numexpr\j+1\relax.center) -- cycle;
        \else
            % Diagonal from top-right to bottom-left
            \fill[PrimaryBlue] (v\i\j.center) -- (v\the\numexpr\i+1\relax\the\numexpr\j+1\relax.center) -- (v\i\the\numexpr\j+1\relax.center) -- cycle;
            \fill[AccentBlue] (v\i\j.center) -- (v\the\numexpr\i+1\relax\the\numexpr\j+1\relax.center) -- (v\the\numexpr\i+1\relax\j.center) -- cycle;
        \fi
    }
}
\end{scope}

\end{tikzpicture}
}
